Generalizing Complex Hypotheses on Product Distributions: Auctions, Prophet Inequalities, and Pandora's Problem

This paper explores a theory of generalization for learning problems on product distributions, complementing the existing learning theories in the sense that it does not rely on any complexity measures of the hypothesis classes. The main contributions are two general sample complexity bounds: (1) $\tilde{O} \big( \frac{nk}{\epsilon^2} \big)$ samples are sufficient and necessary for learning an $\epsilon$-optimal hypothesis in any problem on an $n$-dimensional product distribution, whose marginals have finite supports of sizes at most $k$; (2) $\tilde{O} \big( \frac{n}{\epsilon^2} \big)$ samples are sufficient and necessary for any problem on $n$-dimensional product distributions if it satisfies a notion of strong monotonicity from the algorithmic game theory literature. As applications of these theories, we match the optimal sample complexity for single-parameter revenue maximization (Guo et al., STOC 2019), improve the state-of-the-art for multi-parameter revenue maximization (Gonczarowski and Weinberg, FOCS 2018) and prophet inequality (Correa et al., EC 2019), and provide the first and tight sample complexity bound for Pandora's problem.

==> app-prophet-lb.tex <==
\subsection{Lower Bound}
\label{sec:prophet-lb}

Consider any instance $\vec{D}$.
Recall that for any $0 \le i \le n$, let $\theta_i(\vec{D})$ denote the optimal objective conditioned on not accepting any reward in the first $i$ rounds.
We have:
%
\[
    \theta_0( \vec{D} ) = \opt ( \vec{D} ) 
    \quad,\quad
    \theta_n ( \vec{D} ) = 0 
    ~.
\]

Further, by backward induction, for any $0 \le i < n$ we have:
%
\[
    \theta_{i-1} ( \vec{D} ) = \theta_i( \vec{D} ) + \E_{\type_i \sim D_i} \big[ \big( \type_i - \theta_i ( \vec{D} ) \big)^+ \big] 
    ~.
\]

Intuitively, not taking the reward in round $i$ would be a mistake if $t_i > \theta_i(\vec{D})$, leading to an additive error of $t_i - \theta_i(\vec{D})$;
similarly, taking the reward in round $i$ would be a mistake if $t_i < \theta_i(\vec{D})$, leading to an additive error of $\theta_i(\vec{D}) - t_i$.
Indeed, we first show that the additive error of any algorithm can be decomposed into $n$ parts, where the $i$-th part equals the probability that the algorithm gets to round $i$, i.e., that it does not accept any reward before round $i$, times the expected error compared with the reserve value $\theta_i(\vec{D})$ as defined above.

\begin{lemma}
    \label{lem:prophet-lb-error-decompose}
    Consider any instance $\vec{D}$ and any algorithm.
    Let $Stop_{<i}(\vec{t}_{<i}) = 0$ denote the event that $Stop_j(t_j) = 0$ for all $1 \le j < i$.
    The expected additive error is equal to:
    %
    \[
        \opt(\vec{D}) - \alg(\vec{D}) = \sum_{i=1}^{n} \Pr \big[ Stop_{<i}(\vec{t}_{<i}) = 0 \big] \cdot \E_{\type_i \sim D_i} \big[ \big( \type_i - \theta_i ( \vec{D} ) \big)^+ - \big( \type_i - \theta_i ( \vec{D} ) \big) \cdot Stop_i ( \type_i ) \big]
        ~.
    \]
\end{lemma}

\begin{proof}
    Let $\alg_i ( \vec{D} )$ denote the expected objective by the algorithm conditioned on not accepting any reward in the first $i$ rounds.
    We have for any $1 \le i \le n$:
    %
    \begin{align*}
        \alg_{i-1} ( \vec{D} ) 
        &
        = \alg_i ( \vec{D} ) + \E_{\type_i \sim D_i} \big[ \big( \type_i - \alg_i ( \vec{D} ) \big) \cdot Stop_i ( \type_i ) \big] \\
        &
        = \Pr \big[ Stop_i(\type_i) = 1 \big] \cdot \theta_i ( \vec{D} ) + \Pr \big[ Stop_i(\type_i) = 0 \big] \cdot \alg_i ( \vec{D} ) \\
        &
        \quad + \E_{\type_i \sim D_i} \big[ \big( \type_i - \theta_i ( \vec{D} ) \big) \cdot Stop_i ( \type_i ) \big]
        ~.
    \end{align*}
    
    Therefore, for any $1 \le i \le n$:
    %
    \begin{align*}
        \theta_{i-1}(\vec{D}) - \alg_{i-1} ( \vec{D} ) 
        &
        = \Pr \big[ Stop_i(\type_i) = 0 \big] \cdot \big( \theta_i(\vec{D}) - \alg_i(\vec{D}) \big) \\
        &
        \quad
        + \E_{\type_i \sim D_i} \big[ \big( \type_i - \theta_i ( \vec{D} ) \big)^+ - \big( \type_i - \theta_i ( \vec{D} ) \big) \cdot Stop_i ( \type_i ) \big]
        ~.
    \end{align*}
    
    Solving the recurrence proves the lemma.
\end{proof}

\paragraph{Hard Instances.}
%
We will assume that $n = 2k$ is an even number, and partition the $n$ rounds into $k$ phases, with two rounds in each phase.
Each phase $1 \le i \le k$, has two possible distributions, denoted as $D^+_{2i-1} \times D^+_{2i}$ and $D^-_{2i-1} \times D^-_{2i}$.
Hence, there are $2^k$ instances of concern in total.
Below summarizes the guiding principles of our constructions of the distributions:
%
\begin{enumerate}
    %
    \item For any $0 \le i \le k$, and any instance $\vec{D}$ in the above family:
    %
    \[
        \theta_{2i}(\vec{D}) = \frac{k-i}{2k}
        ~.
    \]
    %
    This invariant allows us to disentangle the construction of distributions in different phases.
    %
    \item 
    %
\end{enumerate}
